Object-Guided Instance Segmentation With Auxiliary Feature Refinement for Biological Images

Instance segmentation is of great importance for many biological applications, such as study of neural cell interactions, plant phenotyping, and quantitatively measuring how cells react to drug treatment. In this paper, we propose a novel box-based instance segmentation method. Box-based instance segmentation methods capture objects via bounding boxes and then perform individual segmentation within each bounding box region. However, existing methods can hardly differentiate the target from its neighboring objects within the same bounding box region due to their similar textures and low-contrast boundaries. To deal with this problem, in this paper, we propose an object-guided instance segmentation method. Our method first detects the center points of the objects, from which the bounding box parameters are then predicted. To perform segmentation, an object-guided coarse-to-fine segmentation branch is built along with the detection branch. The segmentation branch reuses the object features as guidance to separate target object from the neighboring ones within the same bounding box region. To further improve the segmentation quality, we design an auxiliary feature refinement module that densely samples and refines point-wise features in the boundary regions. Experimental results on three biological image datasets demonstrate the advantages of our method. The code will be available at https://github.com/yijingru/ObjGuided-Instance-Segmentation.

==> tables/table1.tex <==
\begin{table*}[t!]
\caption{Instance segmentation evaluation results. AP$_{\{0.5:0.05:0.95\}}$ refers to the averaged AP over 10 IOU thresholds from 0.5 to 0.95 with an interval of 0.05. We intentionally report the AP at three IOU thresholds of 0.5, 0.75 and 0.9. The inference speed FPS (frame per second) is measured on a single RTX 6000 GPU. }
\label{tab1}
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Method & Data & Input Size & AP$^{dec}_{\{0.5:0.05:0.95\}}$& AP$^{seg}_{\{0.5:0.05:0.95\}}$ & AP@0.5 & AP@0.75 & AP@0.9& FPS \\ 
\hline
% neural
DCAN \cite{chen2017dcan}& \multirow{6}{*}{Neural}&$512\times512$& & 10.98&44.82&1.00&0.00&3.55\\
MaskRCNN \cite{he2017mask}&&$800\times800$ & &51.55&94.64&54.43&0.04&15.97\\
PointRend \cite{kirillov2019pointrend}& &$800\times800$&50.93 & 50.61&94.81&50.26&0.07&14.45\\
Ours W.O. Refine& &$512\times512$  & 44.34 &58.26&94.31&67.24&\textbf{3.46}&9.08\\
Ours W. Refine &&$512\times512$   & 44.21 &\textbf{60.38}&\textbf{96.40}&\textbf{72.86}&3.33&9.77\\
\hline
%--------------------------------------------
% plant
DCAN \cite{chen2017dcan}& \multirow{6}{*}{Plant}&$512\times512$ &&16.67&38.86&13.02&0.00&10.90\\
MaskRCNN \cite{he2017mask}&&$800\times 800$&&60.75&90.59&67.31&17.16&17.99\\
%TensorMask \cite{chen2019tensormask} &\\
PointRend \cite{kirillov2019pointrend}& & $800\times 800$& 57.45&59.90 & 90.00& 67.68 & 13.54&16.30\\
Ours W.O. Refine& &$512\times512$ & 59.45 & 74.11 & 92.20 & 79.15& 53.71&8.94\\
Ours W. Refine & & $512\times512$ & 62.99& \textbf{76.71}&\textbf{92.98}&\textbf{81.08} &\textbf{58.25}& 9.03\\
\hline
%-------------------------------------------
% kaggle
DCAN \cite{chen2017dcan}& \multirow{6}{*}{DSB}&$512\times512$& &19.70&48.36&15.56&0.31&1.84\\
MaskRCNN \cite{he2017mask}&&$800\times 800$&&44.20&79.97&44.15&2.84&17.21\\
PointRend \cite{kirillov2019pointrend}& & $800\times 800$& 41.43&43.12 & 80.03& 42.69 & 2.07&14.25\\
Ours W.O. Refine& &$512\times512$&  50.41 & 61.14 & 84.84 & 65.14& \textbf{33.94}&3.47\\
Ours W. Refine & & $512\times512$ &50.95& \textbf{61.25}&\textbf{85.56}& \textbf{65.22} &33.49&3.79\\
\hline
\end{tabular}
\end{table*}
